ChatGPT for GTFS: Benchmarking LLMs on GTFS Understanding and Retrieval

The General Transit Feed Specification (GTFS) standard for publishing transit data is ubiquitous. GTFS being tabular data, with information spread across different files, necessitates specialized tools or packages to retrieve information. Concurrently, the use of Large Language Models(LLMs) for text and information retrieval is growing. The idea of this research is to see if the current widely adopted LLMs (ChatGPT) are able to understand GTFS and retrieve information from GTFS using natural language instructions without explicitly providing information. In this research, we benchmark OpenAI's GPT-3.5-Turbo and GPT-4 LLMs which are the backbone of ChatGPT. ChatGPT demonstrates a reasonable understanding of GTFS by answering 59.7% (GPT-3.5-Turbo) and 73.3% (GPT-4) of our multiple-choice questions (MCQ) correctly. Furthermore, we evaluated the LLMs on information extraction tasks using a filtered GTFS feed containing four routes. We found that program synthesis techniques outperformed zero-shot approaches, achieving up to 93% (90%) accuracy for simple queries and 61% (41%) for complex ones using GPT-4 (GPT-3.5-Turbo).

==> figures/mcq_questions_prompt_none.tex <==
\begin{mdframed}[backgroundcolor=conversationbg, linewidth=0pt]

\begin{systemblock}
You are a helpful assistant with an understanding of GTFS(General Transit Feed Specification).\\
\emph{Instructions:}\\
 - You are given a set of questions with a single correct answer and 4 options a,b,c, and d. \\
 - Choose the option that is most appropriate. Choose \underline{`None of these'} option in case other options are not relevant.\\
  - You do not have to provide any explanation.\\
 - Output only the answer for every question asked. For example, if the correct answer is `a' then output `a'.
\end{systemblock}

\vspace{4pt}
\begin{userblock}
Can a GTFS feed contain multiple agency information? \\a) Each agency should publish a seperate GTFS. \\b) No, GTFS feeds can only represent a single agency.\\ c) None of these\\d) Agencies are not relevant in GTFS feeds.

\end{userblock}
\vspace{4pt}
\begin{assistantblock}
c
\end{assistantblock}
\end{mdframed}


==> tables/dataset.tex <==
\begin{tabular}{|lc|}
\hline
\multicolumn{1}{|l|}{\textbf{Question Type}} & \multicolumn{1}{l|}{\textbf{Number of Questions}} \\ \hline
\multicolumn{2}{|c|}{\textit{GTFS  Understanding}} \\ \hline
\multicolumn{1}{|l|}{Term Definitions}      & 14   \\ \hline
\multicolumn{1}{|l|}{Common Reasoning}      & 28   \\ \hline
\multicolumn{1}{|l|}{File Structure}        & 17   \\ \hline
\multicolumn{1}{|l|}{Attribute Mapping}     & 32   \\ \hline
\multicolumn{1}{|l|}{Data Structure}        & 30   \\ \hline
\multicolumn{1}{|l|}{Categorical Mapping}   & 74   \\ \hline
\multicolumn{2}{|c|}{\textit{GTFS Retrieval}}      \\ \hline
\multicolumn{1}{|l|}{Simple}      & 47   \\ \hline
\multicolumn{1}{|l|}{Complex}      & 41   \\ \hline
\end{tabular}
